MT-SLVR: Multi-Task Self-Supervised Learning for Transformation In(Variant) Representations

Contrastive self-supervised learning has gained attention for its ability to create high-quality representations from large unlabelled data sets. A key reason that these powerful features enable data-efficient learning of downstream tasks is that they provide augmentation invariance, which is often a useful inductive bias. However, the amount and type of invariances preferred is not known apriori, and varies across different downstream tasks. We therefore propose a multi-task self-supervised framework (MT-SLVR) that learns both variant and invariant features in a parameter-efficient manner. Our multi-task representation provides a strong and flexible feature that benefits diverse downstream tasks. We evaluate our approach on few-shot classification tasks drawn from a variety of audio domains and demonstrate improved classification performance on all of them

==> invariances/simsiam_inv.tex <==
    \setlength{\tabcolsep}{4pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1} % Default value: 1
    \begin{table}[h]
    
        \caption{Measured average Mahalanobis distance between original and augmented training (AudioSet) samples for \textbf{SimSiam} based models. As value approaches 0, the model is more invariant to transformation.}
        
        \centering
        \resizebox{\columnwidth}{!}{%
            \begin{tabular}{c|cccccccc|c}
   
			 \toprule
             Model ($f_\theta$) & Head & PS & FD & WN &  MN & TM & TS^1 & TS^2 & Avg\\

             \toprule 

            Cont Only & - & 31.29 & 32.35 & 30.70 & 30.79 & 36.06 & 31.31 & 30.71 & 31.89\\

            \midrule
            
            Pred Only & - & 38.17 & 40.81 & 41.26 & 40.73 & 54.21 & 30.39 & 43.83 & 41.34\\

            \midrule

            MT-Simple & - & 45.00 & 48.15 & 49.76 & 48.06 & 52.30 & 31.86 & 65.70 & 48.69\\

            \midrule
            
            & 0 & 45.00 & 48.51 & 46.53 & 45.69 & 46.23 & 30.37 & 58.78 & 45.87\\
            \multirow{-2}{*}{MT-Split} & 1 & 45.24 & 48.72 & 47.37 & 46.23 & 46.34 & 30.39 & 58.71 & 46.14\\

            \midrule
            
            & 0 & 41.74 & 45.52 & 47.56 & 45.71 & 46.81 & 29.82 & 57.72 & 44.98\\
            \multirow{-2}{*}{MT-Bn} & 1 & 44.17 & 46.98 & 50.54 & 48.75 & 49.35 & 29.84 & 57.19 & 46.69\\

            \midrule
            
            & 0 & 31.37 & 32.11 & 31.63 & 31.63 & 32.19 & 29.64 & 39.46 & 32.58\\
            \multirow{-2}{*}{MT-Series} & 1 & 49.73 & 50.73 & 49.61 & 50.24 & 48.27 & 29.91 & 64.95 & 49.06\\
            
            \midrule
            
            & 0 & 31.64 & 33.20 & 31.77 & 31.81 & 33.25 & 29.95 & 37.25 & 32.7\\
            \multirow{-2}{*}{MT-Parallel} & 1 & 41.20 & 45.44 & 48.09 & 45.16 & 46.38 & 29.94 & 56.02 & 44.6\\

            
             \bottomrule

		    \end{tabular}}
        \label{table:simsiam_inv}
    \end{table}
